The AI-DEC: A Card-based Design Method for User-centered AI Explanations

Increasing evidence suggests that many deployed AI systems do not sufficiently support end-user interaction and information needs. Engaging end-users in the design of these systems can reveal user needs and expectations, yet effective ways of engaging end-users in the AI explanation design remain under-explored. To address this gap, we developed a design method, called AI-DEC, that defines four dimensions of AI explanations that are critical for the integration of AI systems -- communication content, modality, frequency, and direction -- and offers design examples for end-users to design AI explanations that meet their needs. We evaluated this method through co-design sessions with workers in healthcare, finance, and management industries who regularly use AI systems in their daily work. Findings indicate that the AI-DEC effectively supported workers in designing explanations that accommodated diverse levels of performance and autonomy needs, which varied depending on the AI system's workplace role and worker values. We discuss the implications of using the AI-DEC for the user-centered design of AI explanations in real-world systems.

==> figure_AI-DEC_1.tex <==
\begin{figure*}[!h]
  \includegraphics[width=5.5in]{figures/print_1.pdf}
  \caption{\textit{AI-DEC (\textbf{AI} Explanation \textbf{De}sign \textbf{C}ards)} }
  \label{card collection}
%   \vspace{-6pt}
\end{figure*}





==> figure_AI-DEC_2.tex <==
\begin{figure*}[!h]
  \includegraphics[width=5.5in]{figures/print_2.pdf}
  \caption{\textit{AI-DEC (\textbf{AI} Explanation \textbf{De}sign \textbf{C}ards)} }
  \label{card collection}
%   \vspace{-6pt}
\end{figure*}





==> figure_AIDECex.tex <==
\begin{figure*}[!t]
  \includegraphics[width=\textwidth]{figures/ExpStratCards.png}
  \caption{\textit{Explanation Design Cards ---} To help workers generate user-centered explanation designs, we developed \textit{AI-DEC (AI Design Exploration Cards)}. The cards helped workers build structural explanations step by step, expressing their preferences and explainability needs for the automated systems. Based on theories of \textit{communication strategy} \cite{mohr1990communication}, the cards include four facets to constitute explanations: \textit{content}, \textit{modality}, \textit{frequency}, and \textit{direction}. Each of these facets contains design elements that workers can choose from and a design card where workers can input their own design. }
  \label{expCards}
%   \vspace{-6pt}
\end{figure*}



==> figure_teaser.tex <==
\begin{figure*}[!h]
  %\includegraphics[width=\textwidth]{figures/disTeaser.pdf} 
  \includegraphics[width=\textwidth]{figures/teasor2_dis.pdf} 
  \caption{\textit{Using the AI-DEC to Develop Communication Strategies for User-centered AI Explanations ---} 
  We introduce \textit{AI-DEC}, a card-based design method, that involves four critical dimensions for AI explanations: communication content, modality, frequency, and direction. %This method incorporates end-users in crafting tailored AI explanations, enabling them to develop communication strategies aligned with their needs. 
  The figure imitates our co-design session where a worker (\ie end-user) utilizes the AI-DEC to prototype personalized AI explanations meeting their information and interaction requirements.
 %In this work, we have created AI-DEC (Designing AI Explanations for Context) cards, which assist designers in collaborating with end users to develop AI explanations tailored to specific AI use cases. AI-DEC incorporates principles from communication theory and insights from AI and design literature to help users articulate their contextual requirements and propose explanation designs. The figure shows a worker co-designing their communication strategy with an AI practitioner. 
  }
  \label{fig:teasor}
%   \vspace{-6pt}
\end{figure*}

